Efficient and Near-Optimal Online Portfolio Selection

In the problem of online portfolio selection as formulated by Cover (1991), the trader repeatedly distributes her capital over $ d $ assets in each of $ T > 1 $ rounds, with the goal of maximizing the total return. Cover proposed an algorithm, termed Universal Portfolios, that performs nearly as well as the best (in hindsight) static assignment of a portfolio, with an $ O(d\log(T)) $ regret in terms of the logarithmic return. Without imposing any restrictions on the market this guarantee is known to be worst-case optimal, and no other algorithm attaining it has been discovered so far. Unfortunately, Cover's algorithm crucially relies on computing certain $ d $-dimensional integral which must be approximated in any implementation; this results in a prohibitive $ \tilde O(d^4(T+d)^{14}) $ per-round runtime for the fastest known implementation due to Kalai and Vempala (2002). We propose an algorithm for online portfolio selection that admits essentially the same regret guarantee as Universal Portfolios -- up to a constant factor and replacement of $ \log(T) $ with $ \log(T+d) $ -- yet has a drastically reduced runtime of $ \tilde O(d^2(T+d)) $ per round. The selected portfolio minimizes the current logarithmic loss regularized by the log-determinant of its Hessian -- equivalently, the hybrid logarithmic-volumetric barrier of the polytope specified by the asset return vectors. As such, our work reveals surprising connections of online portfolio selection with two classical topics in optimization theory: cutting-plane and interior-point algorithms.

==> conclusion.tex <==
\section*{Conclusion and perspectives}
\label{sec:conclusion}

We have introduced a new algorithm \OurAlgo\ and shown that it enjoys an optimal regret for online portfolio selection. We have also provided an efficient implementation which has a computational complexity $O(d^2 T^2)$. As a technical contribution, we have demonstrate a use of the volumetric regularization in an online learning setting. We think that this tool may have a broader impact in learning theory. To expand this work, we see the following possible ways.
\begin{itemize}
    \item One would be to adapt \OurAlgo\ to natural extensions of online portfolio selection. For example, it may be interesting to take into account transaction costs and/or side information which are crucial in practice \cite{li2018online}.
    \item Another natural follow up would be to design an algorithm even faster than \OurAlgo. Linear computational complexity in $T$ would be ideal like what have been done recently for Ada-BARRONS \cite{zimmert2022pushing}, \cite{mhammedi2022damped}.
    \item From a more theoretical point of view, online portfolio selection is a typical instance of learning with exp-concave functions. We think it is possible generalize our results for any exp-concave losses on the simplex and also on any polytopes. However, the naive extension of our work would probably lead to a multiplicative constant proportional to the number of constraints which may be sub-optimal. An even more interesting challenge is to extend \OurAlgo\ to any exp-concave losses on any convex set. The use of general self-concordant barrier would raise some technical challenges but in case of success would lead to an algorithm competing with ONS in the the full general setting without paying the bound on gradient norms.
    \item Recently, they have been several works trying to design efficient algorithms for logistic regression with logarithmic regret and small multiplicative constant \cite{foster2018logistic}, \cite{jezequel2020efficient}, \cite{agarwal2021efficient}. Despite the efforts, no efficient algorithm with optimal dependence in the radius of the comparative class is known. However, because the mixability of the logistic loss is derived from the exp-concavity of $f(x) = -\log\left(\Pi_{k \in [d]} x_k^{\alpha_k}\right)$ whenever $\alpha_k \ge 0$ and $\sum_{k \in [d]} \alpha_k = 1$, it may be possible to reuse some techniques of this work to design an efficient algorithm with optimal regret.
\end{itemize}
